Testing Poisson Binomial Distributions

A Poisson Binomial distribution over $n$ variables is the distribution of the sum of $n$ independent Bernoullis. We provide a sample near-optimal algorithm for testing whether a distribution $P$ supported on $\{0,...,n\}$ to which we have sample access is a Poisson Binomial distribution, or far from all Poisson Binomial distributions. The sample complexity of our algorithm is $O(n^{1/4})$ to which we provide a matching lower bound. We note that our sample complexity improves quadratically upon that of the naive "learn followed by tolerant-test" approach, while instance optimal identity testing [VV14] is not applicable since we are looking to simultaneously test against a whole family of distributions.

==> abstract.tex <==
\begin{abstract}

Poisson Binomial distributions are sums of independent but not
necessarily identical Bernoulli random variables. 
Given independent samples from a distribution over $[\absz]$, 
we consider the problem of testing if it is a Poisson
Binomial Distribution (\Pbd) or at least $\dst$ far from all \Pbd's. 

It is known that to test if the distribution is \emph{exactly} a
$Binomial(n,1/2)$, or $\dst$ far from it,  requires $O(n^{1/4}/\dst^2)$ samples, and 
to test if it is $\dst$ close or $2\dst$ far requires $O(\sqrt{n}/\log
n)$ samples.  

Exploiting the underlying structure of \Pbd's, 
we provide an algorithm that uses $O(n^{1/4}/\dst^2+1/\dst^6)$
samples. We also provide a lower bound of
$O(n^{1/4}/\dst^2)$ samples. 
\end{abstract}



==> introduction.tex <==
% The introduction goes here
\section{Preliminaries}
Given samples from an unknown distribution over the support $[\absz]$,  
\emph{identity testing} is the problem of deciding if the distribution is 
equal to a \emph{known distribution} or at least $\dst$ away
from it in total variation distance. 

We consider the problem of testing if a distribution is in a 
known class $\cP$ of distributions or is $\dst-$far from it.
 This requires $O(\sqrt{\absz}/\dst^2)$
where $\absz$ is the alphabet size. When $\cP$ contains all
distributions within a distance $\dst/2$ from a known $P$ the problem
is called \emph{Tolerant Identity Testing} and it requires
$\tilde{\Theta}(\absz)$ samples. We consider the problem of testing
against a class of distributions.

\begin{Definition}
A Poisson Binomial Distribution (PBD) over $[\absz]=\{0\upto\absz\}$
is the distribution of $X=\sum_{i=1}^{\absz}X_i$, where each $X_i$ is an
independent Bernoulli random variable. $\pbdabsz$ is the class of all 
Poisson Binomial distributions over $[\absz]$.
\end{Definition} 

\begin{Definition}
The $\ell_1$-distance between $P$ and $Q$ over
$[\absz]$ is $\ellone{P}{Q}\ed \sum_{0\le i\le
  \absz}{|P(i)-Q(i)|}$.
The $\ell_1$-distance between two classes of distributions $\cP$ and
$\cQ$ is $\ellone{\cP}{\cQ}\ed \inf_{P\in\cP,Q\in\cQ}\ellone{P}{Q}$.
\end{Definition} 

{\bf Problem: }
Given samples from an \emph{unknown} distribution $\Pund=(P(0),P(1)\upto P(\absz))$ over
$[\absz]$ determine if $P\in\pbdabsz$ or
$\ellone{\Pund}{\pbdabsz}\ge\dst$.


